Incremental Monoidal Grammars

In this work we define formal grammars in terms of free monoidal categories, along with a functor from the category of formal grammars to the category of automata. Generalising from the Booleans to arbitrary semirings, we extend our construction to weighted formal grammars and weighted automata. This allows us to link the categorical viewpoint on natural language to the standard machine learning notion of probabilistic language model.

==> incremental-discocat.tex <==
%!TEX root = main.tex

\textit{Describe how we can apply the discocat functor on the diagram arrows to map to tensors in Mat. Describe how this can give us semantic information about a partial sentence (in a non-contracted form)}

\textit{Talk about the challenges of comparing/interpreting tensors of different sizes that are formed from applying the discocat functor to different contraction states of the same string. Potentially introduce some approach that allows us to perform this comparison (e.g. frobenius algebra, a ``template tensor'' that we can use to reduce higher order tensors to smaller tensors and preserve relative likelihood, etc)}

\textit{If possible, demonstrate how we can "close the loop" and use the semantic information that discocat provides to improve the quality of our probabilistic modeling (e.g. I shot an elephant in my pajamas). Define the likelihood of a particular diagram (contraction states) based not only on the information about the types and type contractions but also the semantic co-occurrence information that discocat embeddings provide. This may be challenging, but the crux of it is that the resulting tensor from contracting "I" with "in my pajamas" should be larger/more likely than the tensor from contracting "elephant" with "in my pajamas" based on the co-occurrences. Then we can define the probability distribution partially based on this.}

